MVIN: Learning Multiview Items for Recommendation

Researchers have begun to utilize heterogeneous knowledge graphs (KGs) as auxiliary information in recommendation systems to mitigate the cold start and sparsity issues. However, utilizing a graph neural network (GNN) to capture information in KG and further apply in RS is still problematic as it is unable to see each item's properties from multiple perspectives. To address these issues, we propose the multi-view item network (MVIN), a GNN-based recommendation model which provides superior recommendations by describing items from a unique mixed view from user and entity angles. MVIN learns item representations from both the user view and the entity view. From the user view, user-oriented modules score and aggregate features to make recommendations from a personalized perspective constructed according to KG entities which incorporates user click information. From the entity view, the mixing layer contrasts layer-wise GCN information to further obtain comprehensive features from internal entity-entity interactions in the KG. We evaluate MVIN on three real-world datasets: MovieLens-1M (ML-1M), LFM-1b 2015 (LFM-1b), and Amazon-Book (AZ-book). Results show that MVIN significantly outperforms state-of-the-art methods on these three datasets. In addition, from user-view cases, we find that MVIN indeed captures entities that attract users. Figures further illustrate that mixing layers in a heterogeneous KG plays a vital role in neighborhood information aggregation.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> baseline_and_dataset.tex <==
\section{Baseline and Dataset}

In this section, we describe the different baselines in our experiments, after which we describe
our real-world dataset in detail.


\label{sec:baseline}
\subsection{Baseline} \label{Baseline}




\textbf{POP:} a simple but powerful algorithm that uses previous records to compute scores
and recommends the most popular products in the training dataset.


\noindent\textbf{ItemKNN~\cite{1167344}:} this model is one of the most common item-to-item
recommendation models. Each article is taken as an item and the co-occurences of
articles in each session are calculated to recommend articles.

\noindent\textbf{doc2vec~\cite{pmlr-v32-le14}:} a model for learning text representations. We
obtain each article representation by feeding the article content and calculating
the cosine similarities to pick the top-N similar articles for recommendation. Here,
we set the embedding size to 200 and select the learning rate from
\textbraceleft0.1, 0.01, 0.001\textbraceright.

\noindent\textbf{prod2vec~\cite{Grbovic:2015:EYI:2783258.2788627}:} the model learns vector
representations of each article by taking each browsing session as a sequence and
articles within the session as words with skip-gram loss. Prod2vec recommends
articles by computing the cosine similarities between the article representations
and selects the top \textit{N}-similar products. We set the embedding size for items here
to 200. The model is optimized using stochastic gradient ascent, and the learning
rate is selected from \textbraceleft0.1, 0.01, 0.001\textbraceright. The context
neighborhood size for all models was set to 5. We used 20 negative
samples in each vector update.

\noindent\textbf{NARM~\cite{Li:2017:NAS:3132847.3132926}:} a session-based recommendation model
which utilizes the user's main purpose for recommendation; this
purpose
is obtained via attention on previous behaviors within the
session. Here, we set the embedding size to 200. The model is optimized using
Adam with initial learning rates selected from \textbraceleft0.001, 
0.0001\textbraceright; the mini-batch size is fixed at 512.

\noindent\textbf{CDSSM~\cite{a-latent-semantic-model-with-convolutional-pooling-structure-for-information-retrieval}:} the model uses a convolutional neural network to learn low-dimensional semantic vectors followed by multi-layer perceptrons(MLP), after which the normalized dot product is used to calculatethe score between two articles. We here use character embeddings pre-trained with GloVe as word representation. We set the hidden size of final article representation to 128 and embedding size of each word is 50. During training we used the Adam optimizer;
the learning rate was selected from \textbraceleft0.001, 0.0001\textbraceright.

\noindent\textbf{BERT-NN~\cite{devlin2018bert}:} a fine-tuned BERT model. BERT is a new
fine-tuning based representation model that yields state-of-the-art results on
many NLP tasks. We freeze the BERT parameters and use only the final
768-node hidden state on each article followed by a 96-node
FC layer to compute the cosine similarities to pick the top-N similar
articles for recommendation. During training we used the Adam optimizer;
the learning rate was selected from \textbraceleft0.001, 0.0001\textbraceright.

\subsection{Data Preparation}
\label{Data Preparation}

\input{tables/data_statistic.tex}

In our experiments we use two different news websites:
\emph{Pb}, and \emph{Sina}.
\emph{Pb} is a website containing various sports news including basketball,
baseball, and soccer. \emph{Sina} is a general news website with articles ranging from sports, movies, travel, international news, politics, to finance. \footnote{Both datasets will be released upon acceptance.}

For the experiments, our collaborating partner provided a total of three months -- October to December 2018 -- of real-world user logs and news articles. We split the data into three sets: October to November for training, 12/01 to 12/15 for validation, and 12/16 to 12/31 for testing. This setting assesses our method's
ability to handle real-world scenarios, as new articles in the
testing set are mostly unseen in the training and validation sets. 
The total number of articles in each website is listed in Table~\ref{tb:statistic}. 


To construct valid sessions for further experiments 
(see Fig.~\ref{fig:session_example}), we first filter out logs without user cookies. Next, we sort
logs with the same cookie information by view times to form consecutive
article sequences.
We then split the article sequence into different sessions whenever
the time gap exceeds 30 minutes~\cite{Airbnb}. We remove 
repetitive articles in a session as this is usually caused by the user
clicking back to the previous page to search for other articles.
Finally, we remove sessions containing fewer than three articles. 
The statistics and distributions of the two news datasets are shown in
Table~\ref{tb:statistic}, where \emph{news life} is defined as the time period from its
first click to its last click and \emph{cold start ratio} denotes the ratio of
articles observed in the testing set but not in the training set. 



\begin{figure}
    \includegraphics[scale=0.38, trim={0 10 0 -25}]{images/session_construction.png}
    \caption{Constructing valid sessions}
    \label{fig:session_example}
\end{figure}

==> tables/CTR_KGPH_by_nb_size.tex <==

\begin{table}[t]
\small
\centering
\caption{$AUC$ of \system with different size of neighborhoods sampling. We set the size of P set to 16.}
\scalebox{1.0}{
\begin{tabular}{p{2.5cm}|ccccc}
\hline \multicolumn{1}{c|}{\multirow{1}{*}{Size of $K_n$ ($K_m=16$)}} &  \multicolumn{1}{c}{{2}} & \multicolumn{1}{c}{{4}} &
\multicolumn{1}{c}{{8}} & \multicolumn{1}{c}{{16}}&
\multicolumn{1}{c}{{32}} \\ \hline \multicolumn{1}{c|}{ML-1M} & 
\multicolumn{1}{c}{{.9246}} & \multicolumn{1}{c}{{.9257}} &
\multicolumn{1}{c}{{.9245}} & \multicolumn{1}{c}{{.9249}} &
\multicolumn{1}{c}{{.9254}} \\ 
\multicolumn{1}{c|}{LFM-1b}  & 
\multicolumn{1}{c}{{.9428}} & \multicolumn{1}{c}{{.9438}} &
\multicolumn{1}{c}{{.9428}} & \multicolumn{1}{c}{{.9424}} &
\multicolumn{1}{c}{{.9421}} \\
\multicolumn{1}{c|}{AZ-book}  & 
\multicolumn{1}{c}{{.8585}} & \multicolumn{1}{c}{{.8590}} &
\multicolumn{1}{c}{{.8602}} & \multicolumn{1}{c}{{.8573}} &
\multicolumn{1}{c}{{.8574}} \\
\hline
\end{tabular}}
\label{tb:KGPI_by_nb_size}
\end{table}


==> tables/CTR_KGPH_by_wide_hop.tex <==

\begin{table}[t]
\small
\centering
\caption{$AUC$ of \system with different number of hops $H$. Due to hardware constraint we set the sampling size of neighbors to 4.}
\vspace{-0.5 pc}
\scalebox{1.0}{
\begin{tabular}{p{2.5cm}|ccc}
\hline \multicolumn{1}{c|}{\multirow{1}{*}{W hop}} &  \multicolumn{1}{c}{{1}} & \multicolumn{1}{c}{{2}} &
\multicolumn{1}{c}{{3}} \\ \hline \multicolumn{1}{c|}{ML-1M} & 
\multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} &
\multicolumn{1}{c}{{.}}  \\ 
\multicolumn{1}{c|}{LFM-1b}  & 
\multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} &
\multicolumn{1}{c}{{.}}  \\
\multicolumn{1}{c|}{AZ-book}  & 
\multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} &
\multicolumn{1}{c}{{.}}  \\
\hline
\end{tabular}}
\label{tb:KGPH_by_prefernece_hops}
\vspace{-0.5 pc}
\end{table}


==> tables/CTR_KGPI_abla_tmp.tex <==

% \begin{table*}[t]
% \small
% \centering
% \caption{The result 2 of the Ablation study on \system. We shows results of $AUC$ and $ACC$ in CTR prediction on all datasets and it demonstrates the effectiveness of Propagation User Preference, Integration Neighborhoods Information, user clicked items $h^{1}_{i}$, Stage-wise Training, User-Orient transfer, Wide Layer, Deep Layer.}
% \scalebox{1.0}{
% \begin{tabular}{cccccccccccccc}
% \hline
% \multicolumn{8}{c}{Components}&
% \multicolumn{2}{c}{ML-1M}&
% \multicolumn{2}{c}{LFM-1b}&
% \multicolumn{2}{c}{AZ-book} \\
% \cmidrule(lr){1-8}
% \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} 
% \multicolumn{1}{c}{ UP }&
% \multicolumn{1}{c}{ NI }&
% \multicolumn{1}{c}{ CI }&
% \multicolumn{1}{c}{ SW }&
% \multicolumn{1}{c}{ UO(r) }&
% \multicolumn{1}{c}{ UO(e) }&
% \multicolumn{1}{c}{ WL }&
% \multicolumn{1}{c}{ DL }&
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} \\ 
% \hline 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{\textbf{.9318}}} & \multicolumn{1}{c}{{\textbf{.8573}}} & \multicolumn{1}{c}{{\textbf{.9658}}} & \multicolumn{1}{c}{{\textbf{.9112}}} & \multicolumn{1}{c}{{\textbf{.8749}}} & \multicolumn{1}{c}{{\textbf{.7935}}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} &
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & \multicolumn{1}{c}{{}} &  \multicolumn{1}{c}{{}} & \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{.9290}}& \multicolumn{1}{c}{{.8551}} &
% \multicolumn{1}{c}{{.9614}} & \multicolumn{1}{c}{{.9064}} & \multicolumn{1}{c}{{.8647}} & \multicolumn{1}{c}{{.7864}}  \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{.9294}} &
% \multicolumn{1}{c}{{.8554}} & \multicolumn{1}{c}{{.9651}} & \multicolumn{1}{c}{{.9099}} & \multicolumn{1}{c}{{.8626}} & \multicolumn{1}{c}{{.7855}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{.9257}} &
% \multicolumn{1}{c}{{.8503}} & \multicolumn{1}{c}{{.9541}} & \multicolumn{1}{c}{{.8998}} & \multicolumn{1}{c}{{.8608}} & \multicolumn{1}{c}{{.7790}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{.}} &
% \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{.9305}} &
% \multicolumn{1}{c}{{.8565}} & \multicolumn{1}{c}{{.9617}} & \multicolumn{1}{c}{{.9058}} & \multicolumn{1}{c}{{.8672}} & \multicolumn{1}{c}{{.7886}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}}& 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{.9293}} &
% \multicolumn{1}{c}{{.8552}} & \multicolumn{1}{c}{{.9643}} & \multicolumn{1}{c}{{.9084}} & \multicolumn{1}{c}{{.8667}} & \multicolumn{1}{c}{{.7840}} \\
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{.9212}} & \multicolumn{1}{c}{{.8461}} & \multicolumn{1}{c}{{.9190}} & \multicolumn{1}{c}{{.8704}} & \multicolumn{1}{c}{{.7990}} & \multicolumn{1}{c}{{.7277}} \\ 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} 
% \\
% \multicolumn{1}{c}{{}} 
% & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{}} & \multicolumn{1}{c}{{}} & \multicolumn{1}{c}{{.9233}} & \multicolumn{1}{c}{{.8740}} & \multicolumn{1}{c}{{}} & \multicolumn{1}{c}{{}} \\
% \hline
% \end{tabular}}
% \label{tb:KGPI_abla_result_2}
% \end{table*}


% \begin{table*}[t]
% \small
% \centering
% \caption{The result of the Ablation study on \system. We shows results of $AUC$ and $ACC$ in CTR prediction on all datasets and it demonstrates the effectiveness of Propagation User Preference, Integration Neighborhoods Information, user clicked items $h^{1}_{i}$, Stage-wise Training, User-Orient transfer, Wide Layer, Deep Layer.}
% \scalebox{1.0}{
% \begin{tabular}{cccccccccccccc}
% \hline
% \multicolumn{8}{c}{Components}&
% \multicolumn{2}{c}{ML-1M}&
% \multicolumn{2}{c}{LFM-1b}&
% \multicolumn{2}{c}{AZ-book} \\
% \cmidrule(lr){1-8}
% \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} 
% \multicolumn{1}{c}{ UP }&
% \multicolumn{1}{c}{ NI }&
% \multicolumn{1}{c}{ CI }&
% \multicolumn{1}{c}{ SW }&
% \multicolumn{1}{c}{ UO(r) }&
% \multicolumn{1}{c}{ UO(e) }&
% \multicolumn{1}{c}{ WL }&
% \multicolumn{1}{c}{ DL }&
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} \\ 
% \hline 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{\textbf{.9318}}} & \multicolumn{1}{c}{{\textbf{.8573}}} & \multicolumn{1}{c}{{\textbf{.9658}}} & \multicolumn{1}{c}{{\textbf{.9112}}} & \multicolumn{1}{c}{{\textbf{.8749}}} & \multicolumn{1}{c}{{\textbf{.7935}}} \\
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{.9212}} & \multicolumn{1}{c}{{.8461}} & \multicolumn{1}{c}{{.9190}} & \multicolumn{1}{c}{{.8704}} & \multicolumn{1}{c}{{.7990}} & \multicolumn{1}{c}{{.7277}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} &
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{.9290}}& \multicolumn{1}{c}{{.8551}} &
% \multicolumn{1}{c}{{.9614}} & \multicolumn{1}{c}{{.9064}} & \multicolumn{1}{c}{{.8647}} & \multicolumn{1}{c}{{.7864}}  \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{.9294}} &
% \multicolumn{1}{c}{{.8554}} & \multicolumn{1}{c}{{.9651}} & \multicolumn{1}{c}{{.9099}} & \multicolumn{1}{c}{{.8626}} & \multicolumn{1}{c}{{.7855}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} &  \multicolumn{1}{c}{{.9257}} &
% \multicolumn{1}{c}{{.8503}} & \multicolumn{1}{c}{{.9541}} & \multicolumn{1}{c}{{.8998}} & \multicolumn{1}{c}{{.8608}} & \multicolumn{1}{c}{{.7790}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{.9305}} &
% \multicolumn{1}{c}{{.8565}} & \multicolumn{1}{c}{{.9617}} & \multicolumn{1}{c}{{.9058}} & \multicolumn{1}{c}{{.8672}} & \multicolumn{1}{c}{{.7886}} \\
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}}& 
% \multicolumn{1}{c}{{}} & 
% \multicolumn{1}{c}{{{\color{blue} \CheckmarkBold}}} & \multicolumn{1}{c}{{.9293}} &
% \multicolumn{1}{c}{{.8552}} & \multicolumn{1}{c}{{.9643}} & \multicolumn{1}{c}{{.9084}} & \multicolumn{1}{c}{{.8683}} & \multicolumn{1}{c}{{.7857}} \\
% \hline
% \end{tabular}}
% \label{tb:KGPI_abla_result}
% \end{table*}


% \begin{table*}[t]
% \small
% \centering
% \caption{The results of $AUC$ and $ACC$ in CTR prediction on all datasets}
% \scalebox{1.0}{
% \begin{tabular}{ccccccc}
% \hline \multicolumn{1}{c}{\multirow{2}{*}{Model}} &
% \multicolumn{2}{c}{ML-1M}&
% \multicolumn{2}{c}{LFM-1b}&
% \multicolumn{2}{c}{AZ-book} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} \\ 
% \hline 
% \multicolumn{1}{c}{{\system-P}} & \multicolumn{1}{c}{{.9290}}& \multicolumn{1}{c}{{.8551}} &
% \multicolumn{1}{c}{{.9614}} & \multicolumn{1}{c}{{.9064}} & \multicolumn{1}{c}{{.8647}} & \multicolumn{1}{c}{{.7864}}  \\
% \multicolumn{1}{c}{{\system-N}}
% & \multicolumn{1}{c}{{.9212}} & \multicolumn{1}{c}{{.8461}} & \multicolumn{1}{c}{{.9190}} & \multicolumn{1}{c}{{.8704}} & \multicolumn{1}{c}{{.7990}} & \multicolumn{1}{c}{{.7277}} \\
% \multicolumn{1}{c}{\system-w/o $h^{1}_{i}$}& \multicolumn{1}{c}{{.9294}} &
% \multicolumn{1}{c}{{.8554}} & \multicolumn{1}{c}{{.9651}} & \multicolumn{1}{c}{{.9099}} & \multicolumn{1}{c}{{.8626}} & \multicolumn{1}{c}{{.7855}} \\
% \multicolumn{1}{c}{{\system-w/o SW}} & \multicolumn{1}{c}{{.9257}} &
% \multicolumn{1}{c}{{.8503}} & \multicolumn{1}{c}{{.9541}} & \multicolumn{1}{c}{{.8998}} & \multicolumn{1}{c}{{.8608}} & \multicolumn{1}{c}{{.7790}} \\
% \multicolumn{1}{c}{{\system-w/o user orient}}& \multicolumn{1}{c}{{.9305}} &
% \multicolumn{1}{c}{{.8565}} & \multicolumn{1}{c}{{.9617}} & \multicolumn{1}{c}{{.9058}} & \multicolumn{1}{c}{{.8672}} & \multicolumn{1}{c}{{.7886}} \\
% \multicolumn{1}{c}{{\system-w/o wide layer}}& \multicolumn{1}{c}{{.9293}} &
% \multicolumn{1}{c}{{.8552}} & \multicolumn{1}{c}{{.9643}} & \multicolumn{1}{c}{{.9084}} & \multicolumn{1}{c}{{.8683}} & \multicolumn{1}{c}{{.7857}} \\
% \hline
% \end{tabular}}
% \label{tb:KGPI_abla_result}
% \end{table*}




% \begin{table*}[t]
% \small
% \centering
% \caption{The results of $AUC$ and $ACC$ in CTR prediction on all datasets}
% \scalebox{1.0}{
% \begin{tabular}{ccccccc}
% \hline \multicolumn{1}{c}{\multirow{2}{*}{Model}} &
% \multicolumn{2}{c}{MovieLens-1M}&
% \multicolumn{2}{c}{LFM-1b 2015}&
% \multicolumn{2}{c}{Amazon-book} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} &
% \multicolumn{1}{c}{\emph{AUC}} & \multicolumn{1}{c}{\emph{ACC}} \\ 
% \hline
% \multicolumn{1}{c}{{w/o SW}} & \multicolumn{1}{c}{{.9265}} &
% \multicolumn{1}{c}{{.8524}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}}  \\
% \multicolumn{1}{c}{{w/o user orient}}& \multicolumn{1}{c}{{.9263}} &
% \multicolumn{1}{c}{{.8525}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}}  \\
% \multicolumn{1}{c}{{w/o user clicked item $h^{1}_{i}$}}& \multicolumn{1}{c}{{.9232}} &
% \multicolumn{1}{c}{{.8485}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{}}  \\
% \multicolumn{1}{c}{{w/o wide\&deep}}& \multicolumn{1}{c}{{.9187}} &
% \multicolumn{1}{c}{{.8434}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} \\
% \multicolumn{1}{c}{{w/o HO Neighborhoods}} & \multicolumn{1}{c}{{.9242}}& \multicolumn{1}{c}{{.8491}} &
% \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}}  \\
% \multicolumn{1}{c}{{w/o User preference}}
% & \multicolumn{1}{c}{{.9156}} & \multicolumn{1}{c}{{.8406}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}}  \\

% \hline
% \end{tabular}}
% \label{tb:KGPH_CTR_result}
% \end{table*}





==> tables/KGPI_parameter.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|ccc}  \hline & ML-1M & LFM-1b & AZ-book \\ \hline
S_p & 64 & 64 & 16 \\ 
S_i & 4 & 8 & 8 \\
d & 16 & 16 & 16 \\
P hop & 2 & 2 & 1 \\
W hop & 1 & 1 & 2 \\
D hop & 1 & 2 & 2 \\
\lambda & 1e-7 & 2e-7 & 5e-7 \\
\eta & 5e-3 & 4e-3 & 5e-3 \\
\hline 
\end{tabular}
\caption{\system hyper-parameter settings for three datasets, where d is entity embedding and relation dimension, $\lambda$ is the entropy regularization constant, $\eta$ is the learning rate and P, W, D hop are the number of preference set, wide and deep hop, respectively.}
\label{tb:parameter}
\end{table}

==> tables/Top_k_RippleNet_KGCN.tex <==

\begin{table*}[t]
\small
\centering
\caption{$Recall@K$ in top-K recommendation on all
datasets}
\scalebox{1.0}{
\begin{tabular}{p{1.8cm}|cc|cc|cc|cc|cc|cc}
\hline \multicolumn{1}{c|}{\multirow{2}{*}{Model}} &
\multicolumn{2}{c|}{MovieLens-1M} &
\multicolumn{2}{c|}{Book-Crossing} &
\multicolumn{2}{c|}{Last.FM 2011} &
\multicolumn{2}{c|}{LFM-1b 2015} &
\multicolumn{2}{c|}{Amazon-book} &
\multicolumn{2}{c}{Yelp 2018} \\
    & \multicolumn{1}{c}{\emph{R@25}} & \multicolumn{1}{c|}{\emph{R@50}} &
\multicolumn{1}{c}{\emph{R@25}} & \multicolumn{1}{c|}{\emph{R@50}} &
\multicolumn{1}{c}{\emph{R@25}} & \multicolumn{1}{c|}{\emph{R@50}} &
\multicolumn{1}{c}{\emph{R@25}} & \multicolumn{1}{c|}{\emph{R@50}} &
\multicolumn{1}{c}{\emph{R@25}} & \multicolumn{1}{c|}{\emph{R@50}} &
\multicolumn{1}{c}{\emph{R@25}} & \multicolumn{1}{c}{\emph{R@50}} \\  \hline 
\multicolumn{1}{c|}{{KGNN}} & \multicolumn{1}{c}{{.1229}} &
\multicolumn{1}{c|}{{.2102}} & \multicolumn{1}{c}{{.0483}} & \multicolumn{1}{c|}{{.0763}} & \multicolumn{1}{c}{{.1343}} & \multicolumn{1}{c|}{{.1890}} & \multicolumn{1}{c}{{.0067}} & \multicolumn{1}{c|}{{.0121}} & \multicolumn{1}{c}{{.0377}} & \multicolumn{1}{c|}{{.0603}} & \multicolumn{1}{c}{{.0395}} & \multicolumn{1}{c}{{.0634}} \\
\multicolumn{1}{c|}{{KGNN-SW}} & \multicolumn{1}{c}{{.1308}} &
\multicolumn{1}{c|}{{.2236}} & \multicolumn{1}{c}{{.0478}} & \multicolumn{1}{c|}{{.0785}} & \multicolumn{1}{c}{{.1463}} & \multicolumn{1}{c|}{{.2119}} & \multicolumn{1}{c}{{.0079}} & \multicolumn{1}{c|}{{.0134}} & \multicolumn{1}{c}{{.0405}} & \multicolumn{1}{c|}{{.0672}} & \multicolumn{1}{c}{{.0412}} & \multicolumn{1}{c}{{.0679}} \\
\multicolumn{1}{c|}{{RippleNet}} & \multicolumn{1}{c}{{.1302}} &
\multicolumn{1}{c|}{{.2300}} & \multicolumn{1}{c}{{.0482}} & \multicolumn{1}{c|}{{.0792}} & \multicolumn{1}{c}{{.1177}} & \multicolumn{1}{c|}{{.1917}} & \multicolumn{1}{c}{{.0101}} & \multicolumn{1}{c|}{{.0173}} & \multicolumn{1}{c}{{.0362}} & \multicolumn{1}{c|}{{.0618}} & \multicolumn{1}{c}{{.0400}} & \multicolumn{1}{c}{{.0692}} \\
\multicolumn{1}{c|}{{RippleNet-SW}} & \multicolumn{1}{c}{{.1339}} &
\multicolumn{1}{c|}{{.2371}} & \multicolumn{1}{c}{{.0491}} & \multicolumn{1}{c|}{{.0797}} & \multicolumn{1}{c}{{.1158}} & \multicolumn{1}{c|}{{.1917}} & \multicolumn{1}{c}{{.0123}} & \multicolumn{1}{c|}{{.0182}} & \multicolumn{1}{c}{{.0578}} & \multicolumn{1}{c|}{{.0910}} & \multicolumn{1}{c}{{.0509}} & \multicolumn{1}{c}{{.0853}} \\ 
\hline
\end{tabular}}
\label{tb:KGNN_top_k_result}
\end{table*}
